Towards hyperparameter-free optimization with differential privacy

Differential privacy (DP) is a privacy-preserving paradigm that protects the training data when training deep learning models. Critically, the performance of models is determined by the training hyperparameters, especially those of the learning rate schedule, thus requiring fine-grained hyperparameter tuning on the data. In practice, it is common to tune the learning rate hyperparameters through the grid search that (1) is computationally expensive as multiple runs are needed, and (2) increases the risk of data leakage as the selection of hyperparameters is data-dependent. In this work, we adapt the automatic learning rate schedule to DP optimization for any models and optimizers, so as to significantly mitigate or even eliminate the cost of hyperparameter tuning when applied together with automatic per-sample gradient clipping. Our hyperparameter-free DP optimization is almost as computationally efficient as the standard non-DP optimization, and achieves state-of-the-art DP performance on various language and vision tasks.

==> src/zhiqi_try.tex <==
import torch
import numpy as np
import copy
import torch.nn.functional as F
from scipy.optimize import curve_fit
from torch.optim.lr_scheduler import LRScheduler

def fit_func2(x, a, b):
    return a * x**2 + b * x

class LrAdapter():
    def __init__(self, configs, mini_bs):
        self.lr_tracker = []
        self.mini_bs = mini_bs
        self.criterion = self.get_criterion()
        for k, v in configs.items():
            setattr(self, k, v)
            
    def get_criterion(self):
        raise NotImplementedError
            
    def get_batch(self, tr_iter, device):
        raise NotImplementedError
    
    def get_loss(self, net, batch):
        raise NotImplementedError
    
    def adjust_alg1(self, net, optimizer, basic_lr, inner_steps=1, tr_iter=None, noise_multiplier=None, device=None, scale=1.0):
        # lr_adapter.adjust_alg1(net, optimizer, args.lr, n_acc_steps, tr_iter, noise_multiplier, device)
        existing_lr = optimizer.param_groups[0]['lr']
        for param in net.parameters():
            if param.requires_grad:
                param.previous = param.data.clone()
        optimizer.step() # will recover latter
        
        total_phi_norm = 0.0
        for param in net.parameters():
            if param.requires_grad:
                param.phi = (param.previous-param.data).clone()/existing_lr # g_priv
                total_phi_norm += torch.norm(param.phi).item()
                
        with torch.no_grad():
            lr_list = np.array([self.est_unit*existing_lr, -self.est_unit*existing_lr, 0])
            loss_list = np.zeros_like(lr_list)
            
            for _ in range(inner_steps):
                batch = self.get_batch(tr_iter, device)
                for lr_idx, lr in enumerate(lr_list):
                    # set parameters
                    for param in net.parameters():
                        if param.requires_grad:
                            param.data = param.previous - lr*param.phi
                    
                    # get loss
                    loss_temp = self.get_loss(net, batch)
                    loss_temp = torch.clamp(loss_temp, 0, self.loss_thre).sum()
                    
                    loss_list[lr_idx] += loss_temp.item()
            
            for lr_idx, lr in enumerate(lr_list):
                if noise_multiplier is not None:
                    loss_list[lr_idx] += noise_multiplier*self.loss_thre*torch.randn(1).to(device).item()
                loss_list[lr_idx] /= (self.mini_bs * inner_steps)

            if self.ada_thre:
                self.loss_thre = loss_list.sum()
            
            try:
                [a, b] = curve_fit(fit_func2, lr_list, loss_list-loss_list[-1])[0]
                
                # if a < 0 or b > 0:
                    # print('=====',a,b)
                    # temp_lr=optimizer.param_groups[0]['lr']
                # else:
                    # temp_lr=-b/a*0.5 # |G|^2 / G^\top H G
                if b < 0:
                    temp_lr = -b * basic_lr / total_phi_norm**2
                    print(f"===== {total_phi_norm} | {-b}")
                else:
                    print('=====',a,b)
                    temp_lr=optimizer.param_groups[0]['lr']
                    
                for g in optimizer.param_groups:
                    # tmp = max(min(temp_lr,g['lr']*self.lr_range_scale),g['lr']/self.lr_range_scale) * (1-self.lr_coeff) * scale + g['lr'] * self.lr_coeff
                    tmp = max(min(temp_lr,g['lr']*self.lr_range_scale),g['lr']/self.lr_range_scale) * (1-self.lr_coeff) + g['lr'] * self.lr_coeff
                    # tmp = temp_lr
                    g['lr'] = tmp
            except:
                pass
        self.lr_tracker.append(optimizer.param_groups[0]['lr'])
        
    def adjust_alg11(self, net, optimizer, basic_lr, inner_steps=1, tr_iter=None, noise_multiplier=None, device=None, scale=1.0):
        existing_lr = optimizer.param_groups[0]['lr']
        for param in net.parameters():
            if param.requires_grad:
                param.previous = param.data.clone()
        optimizer.step() # will recover latter
        
        total_phi_norm = 0.0
        for param in net.parameters():
            if param.requires_grad:
                param.phi = (param.previous-param.data).clone()/existing_lr # g_priv
                total_phi_norm += torch.norm(param.phi).item()
                
        with torch.no_grad():
            lr_list = np.array([self.est_unit*existing_lr, -self.est_unit*existing_lr, 0])
            loss_list = np.zeros_like(lr_list)
            
            for _ in range(inner_steps):
                batch = self.get_batch(tr_iter, device)
                for lr_idx, lr in enumerate(lr_list):
                    # set parameters
                    for param in net.parameters():
                        if param.requires_grad:
                            param.data = param.previous - lr*param.phi
                    
                    # get loss
                    loss_temp = self.get_loss(net, batch)
                    loss_temp = torch.clamp(loss_temp, 0, self.loss_thre).sum()
                    
                    loss_list[lr_idx] += loss_temp.item()
            
            for lr_idx, lr in enumerate(lr_list):
                if noise_multiplier is not None:
                    loss_list[lr_idx] += noise_multiplier*self.loss_thre*torch.randn(1).to(device).item()
                loss_list[lr_idx] /= (self.mini_bs * inner_steps)

            if self.ada_thre:
                self.loss_thre = loss_list.sum()
            
            try:
                [a, b] = curve_fit(fit_func2, lr_list, loss_list-loss_list[-1])[0]
                
                # if a < 0 or b > 0:
                    # print('=====',a,b)
                    # temp_lr=optimizer.param_groups[0]['lr']
                # else:
                    # temp_lr=-b/a*0.5 # |G|^2 / G^\top H G
                if b < 0:
                    temp_lr = -b * basic_lr
                    print(f"===== {-b}")
                else:
                    print('=====',a,b)
                    temp_lr=optimizer.param_groups[0]['lr']
                    
                for g in optimizer.param_groups:
                    # tmp = max(min(temp_lr,g['lr']*self.lr_range_scale),g['lr']/self.lr_range_scale) * (1-self.lr_coeff) * scale + g['lr'] * self.lr_coeff
                    tmp = max(min(temp_lr,g['lr']*self.lr_range_scale),g['lr']/self.lr_range_scale) * (1-self.lr_coeff) * scale + g['lr'] * self.lr_coeff
                    # tmp = temp_lr
                    g['lr'] = tmp
            except:
                pass
        self.lr_tracker.append(optimizer.param_groups[0]['lr'])
            
    def adjust(self, net, optimizer, inner_steps=1, tr_iter=None, noise_multiplier=None, device=None, scale=1.0):
        if hasattr(self, 'sigma'):
            noise_multiplier = self.sigma
        existing_lr = optimizer.param_groups[0]['lr']
        for param in net.parameters():
            if param.requires_grad:
                param.previous = param.data.clone()
        optimizer.step() # will recover latter
        for param in net.parameters():
            if param.requires_grad:
                param.phi = (param.previous-param.data).clone()/existing_lr # g_priv
                
        with torch.no_grad():
            lr_list = np.array([-2*existing_lr,-existing_lr,2*existing_lr, existing_lr, 0])
            loss_list = np.zeros_like(lr_list)
            
            for _ in range(inner_steps):
                batch = self.get_batch(tr_iter, device)
                for lr_idx, lr in enumerate(lr_list):
                    # set parameters
                    for param in net.parameters():
                        if param.requires_grad:
                            param.data = param.previous - lr*param.phi

                    # get loss
                    try:
                        loss_temp = self.get_loss(net, batch)
                    except:
                        import pdb; pdb.set_trace()
                    loss_temp = torch.clamp(loss_temp, 0, self.loss_thre).sum()
                    loss_temp = loss_temp.sum()
                    
                    loss_list[lr_idx] += loss_temp.item()
            
            for lr_idx, lr in enumerate(lr_list):
                if noise_multiplier is not None:
                    loss_list[lr_idx] += noise_multiplier*self.loss_thre*torch.randn(1).to(device).item()
                loss_list[lr_idx] /= (self.mini_bs * inner_steps)

            if self.ada_thre:
                self.loss_thre = loss_list.sum()
            
            try:
                [gHg, Gg] = curve_fit(fit_func2, lr_list, loss_list-loss_list[-1])[0]
                
                # if gHg < 0 or Gg > 0:
                #     print('=====',gHg,Gg)
                #     temp_lr=optimizer.param_groups[0]['lr']
                # else:
                #     temp_lr=-Gg/gHg*0.5 # |G|^2 / G^\top H G
                
                if gHg < 0 or Gg > 0:
                    print('===== [pass]',gHg,Gg)
                    print(f"{list(lr_list)},{loss_list}")
                    temp_lr=optimizer.param_groups[0]['lr']*scale # TODO:for gpt
                else:
                    print(loss_list[-1],'=====',gHg,Gg,-Gg/gHg*0.5,optimizer.param_groups[0]['lr'])
                    temp_lr=-Gg/gHg*0.5 # |G|^2 / G^\top H G
                    
                for g in optimizer.param_groups:
                    tmp = min(temp_lr,g['lr']*self.lr_range_scale) * (1-self.lr_coeff) * scale + g['lr'] * self.lr_coeff
                    if not hasattr(self, 'min_auto_lr'):
                        self.min_auto_lr = tmp
                    elif tmp < self.min_auto_lr:
                        self.min_auto_lr = tmp
                    if tmp < g['lr'] and self.set_min:
                        g['lr'] = self.min_auto_lr
                    else:
                        g['lr'] = tmp
            except:
                pass
        self.lr_tracker.append(optimizer.param_groups[0]['lr'])
        
    def adjust_plot(self, net, optimizer, inner_steps=1, tr_iter=None, noise_multiplier=None, device=None, scale=1.0, print_curve=False):
        if hasattr(self, 'sigma'):
            noise_multiplier = self.sigma
        existing_lr = optimizer.param_groups[0]['lr']
        for param in net.parameters():
            if param.requires_grad:
                param.previous = param.data.clone()
        optimizer.step() # will recover latter
        for param in net.parameters():
            if param.requires_grad:
                param.phi = (param.previous-param.data).clone()/existing_lr # g_priv
                
        with torch.no_grad():
            # lr_list = np.array([self.est_unit*existing_lr*10, self.est_unit*existing_lr*2, self.est_unit*existing_lr, -self.est_unit*existing_lr, -2*self.est_unit*existing_lr, -10*self.est_unit*existing_lr, 0])
            lr_list = np.array([2*self.est_unit*existing_lr, -2*self.est_unit*existing_lr, existing_lr, -existing_lr, 0])
            # lr_list = np.array([2*existing_lr, -2*existing_lr, existing_lr, -existing_lr, 0])
            loss_list = np.zeros_like(lr_list)
            loss_list_nocn = np.zeros_like(loss_list)
            
            for _ in range(inner_steps):
                batch = self.get_batch(tr_iter, device)
                for lr_idx, lr in enumerate(lr_list):
                    # set parameters
                    for param in net.parameters():
                        if param.requires_grad:
                            param.data = param.previous - lr*param.phi

                    # get loss
                    loss_temp = self.get_loss(net, batch)
                    loss_temp_ = torch.clamp(loss_temp, 0, self.loss_thre).sum()
                    
                    loss_list[lr_idx] += loss_temp_.item()
                    loss_list_nocn[lr_idx] += loss_temp.sum().item()
            
            loss_list_c = copy.deepcopy(loss_list)
            gn_list = np.zeros_like(lr_list)
            # ln_list = np.zeros_like(lr_list)
            for lr_idx, lr in enumerate(lr_list):
                # clipped
                loss_list[lr_idx] /= (self.mini_bs * inner_steps)
                loss_list_c[lr_idx] /= (self.mini_bs * inner_steps)
                
                # no-clipped
                loss_list_nocn[lr_idx] /= (self.mini_bs * inner_steps)
                
                # gaussian noise
                gn = noise_multiplier*self.loss_thre*torch.randn(1).to(device).item() / (self.mini_bs * inner_steps)
                
                # laplacian noise
                # ln = xxx / (self.mini_bs * inner_steps)
                
                loss_list[lr_idx] += gn
                gn_list[lr_idx] = gn
                # ln_list[lr_idx] = ln

            if self.ada_thre:
                self.loss_thre = loss_list.sum()
            
            try:
                [gHg, Gg] = curve_fit(fit_func2, lr_list, loss_list-loss_list[-1])[0]
                
                if gHg < 0 or Gg > 0:
                    print('=====',gHg,Gg)
                    temp_lr=optimizer.param_groups[0]['lr']
                else:
                    temp_lr=-Gg/gHg*0.5 # |G|^2 / G^\top H G
                    
                for g in optimizer.param_groups:
                    tmp = max(min(temp_lr,g['lr']*self.lr_range_scale),g['lr']/self.lr_range_scale) * (1-self.lr_coeff) * scale + g['lr'] * self.lr_coeff
                    if not hasattr(self, 'min_auto_lr'):
                        self.min_auto_lr = tmp
                    elif tmp < self.min_auto_lr:
                        self.min_auto_lr = tmp
                    if tmp < g['lr'] and self.set_min:
                        g['lr'] = self.min_auto_lr
                    else:
                        g['lr'] = tmp
            except:
                gHg = 0
                Gg = 0
                pass
            if print_curve:
                print("AUTO-PLOT")
                print(lr_list.tolist())
                print(loss_list_nocn.tolist())
                print(loss_list_c.tolist())
                print(loss_list.tolist())
                print(gn_list.tolist())
                print(gHg, Gg)
                # print(ln_list.tolist())
                
        self.lr_tracker.append(optimizer.param_groups[0]['lr'])
        
    def adjust_diff(self, net, optimizer, inner_steps=1, tr_iter=None, noise_multiplier=None):
        device = net.device
        existing_lr = optimizer.param_groups[0]['lr']
        for param in net.parameters():
            if param.requires_grad:
                param.previous = param.data.clone()
        optimizer.step() # will recover latter
        for param in net.parameters():
            if param.requires_grad:
                param.phi = (param.previous-param.data).clone()/existing_lr # g_priv
                
        with torch.no_grad():
            lr_list = np.array([existing_lr, -existing_lr, 0])
            loss_list = np.zeros_like(lr_list)
            
            for _ in range(inner_steps):
                batch = self.get_batch(tr_iter, device)
                for lr_idx, lr in enumerate(lr_list):
                    # set parameters
                    for param in net.parameters():
                        if param.requires_grad:
                            param.data = param.previous - lr*param.phi
                    
                    # get loss
                    loss_temp = self.get_loss(net, batch)
                    loss_temp = torch.clamp(loss_temp, 0, self.loss_thre).sum()
                    
                    loss_list[lr_idx] += loss_temp.item()
            
            for lr_idx, lr in enumerate(lr_list):
                if noise_multiplier is not None:
                    loss_list[lr_idx] += noise_multiplier*self.loss_thre*torch.randn(1).to(device).item()
                loss_list[lr_idx] /= (self.mini_bs * inner_steps)
            if self.ada_thre:
                self.loss_thre = loss_list.sum()
            
            try:
                temp_lr = (loss_list[0]-loss_list[1]) / (loss_list[0] + loss_list[1] - 2*loss_list[-1])

                for g in optimizer.param_groups:
                    if temp_lr > 0:
                        g['lr'] = max(min(temp_lr,g['lr']*self.lr_range_scale),g['lr']/self.lr_range_scale) * (1-self.lr_coeff) + g['lr'] * self.lr_coeff
            except:
                pass

        self.lr_tracker.append(optimizer.param_groups[0]['lr'])

            
class LrAdapter_CV(LrAdapter):
    def __init__(self, configs, mini_bs):
        super().__init__(configs, mini_bs)
        
    def get_criterion(self):
        return torch.nn.CrossEntropyLoss(reduction='none')
    
    def get_batch(self, tr_iter, device):
        inputs, targets = next(tr_iter)
        inputs, targets = inputs.to(device), targets.to(device)
        return (inputs, targets)
    
    def get_loss(self, net, batch):
        inputs, targets = batch
        outputs = net(inputs)
        loss_temp = self.criterion(outputs, targets)
        return loss_temp
            
class LrAdapter_NLU(LrAdapter):
    def __init__(self, configs, mini_bs, trainer):
        super().__init__(configs, mini_bs)
        self.trainer = trainer
        
    def get_criterion(self):
        return None
    
    def get_batch(self, tr_iter, device):
        inputs = next(tr_iter)
        return self.trainer._prepare_inputs(inputs)
    
    def get_loss(self, net, batch):
        return self.trainer.compute_loss(net, batch)
    
class LrAdapter_NLG(LrAdapter):
    def __init__(self, configs, mini_bs, trainer):
        super().__init__(configs, mini_bs)
        self.trainer = trainer
        
    def get_criterion(self):
        return None
    
    def get_batch(self, tr_iter, device):
        inputs = next(tr_iter)
        return self.trainer._prepare_inputs(inputs)
    
    def get_loss(self, net, batch):
        return self.trainer.compute_loss(net, batch)
    
class AutoScheduler(LRScheduler):
    def __init__(self, optimizer, configs, mini_bs, trainer, last_step=-1, verbose=False):
        self.lr_adapter = LrAdapter_NLU(configs, mini_bs, trainer)
        self.lazy_freq = configs['lazy_freq']
        self.step_count = 0  # Initialize step count
        super().__init__(optimizer, last_epoch=last_step, verbose=verbose)

    def get_lr(self):
        return self._last_lr
    
    def _initial_step(self):
        """Initialize step counts and performs a step"""
        self.optimizer._step_count = 0
        self._step_count = 0
        # self.step()
        self._last_lr = [g['lr'] for g in self.optimizer.param_groups]

    def step(self, net, inner_steps, tr_iter, noise_multiplier=None, device=None):
        """Perform a scheduler step only after lazy_freq optimizer updates."""
        # Increment internal step count
        self.step_count += 1
        
        if self.step_count % self.lazy_freq == 0:
            self.lr_adapter.adjust(net, self.optimizer, inner_steps, tr_iter, noise_multiplier, device)
            self._last_lr = [g['lr'] for g in self.optimizer.param_groups]


from autodp.mechanism_zoo import NoisySGD_Mechanism,SubsampleGaussianMechanism
from autodp.calibrator_zoo import generalized_eps_delta_calibrator
from opacus.accountants.utils import get_noise_multiplier #version>1.0
from scipy.optimize import *
from autodp.transformer_zoo import Composition

import numpy as np
import warnings
warnings.filterwarnings("ignore")


def get_sigma(
    epochs,
    epsilon,
    delta,
    sample_rate,
    accountant='rdp',
):
    if accountant == 'rdp':
        general_calibrate=generalized_eps_delta_calibrator()
        params = {}
        params['prob'] = sample_rate
        params['sigma'] = None
        params['coeff'] = int(epochs/sample_rate)
        mech4 = general_calibrate(SubsampleGaussianMechanism, epsilon, delta, [0,10],params=params,para_name='sigma', name='Subsampled_Gaussian')
        #print(mech4.name, mech4.params, mech4.get_approxDP(delta))
        sigma=mech4.params['sigma']
        print(f"AutoDP sigma: {sigma}")
    elif accountant == 'gdp':
        sigma=get_noise_multiplier(
                        target_epsilon = epsilon,
                        target_delta = delta,
                        sample_rate = batch_sizsample_rate,
                        epochs = epochs,
                        accountant='gdp'
        )
        print(f'Opacus GDP sigma: {sigma}')
    else:
        raise ValueError
    return sigma


def find_c(eps, 
           delta,
           sigma, 
           epochs,
           sample_rate, 
           forward_cnt,
           frequency,
           sigma_coeff=1.01,
           ):
    def eps_from_c(c):
        gradMechanism=NoisySGD_Mechanism(prob=sample_rate, 
                                        sigma=sigma_coeff*sigma,
                                        niter=int(epochs/sample_rate)
                                        )
        lossMechanism=NoisySGD_Mechanism(prob=sample_rate, 
                                         sigma=c,
                                         niter=int(forward_cnt*epochs/sample_rate/frequency)
                                         ) 
        #https://github.com/yuxiangw/autodp/blob/master/example/example_composition.py
        compose = Composition()
        composed_mech = compose([gradMechanism, lossMechanism], [1, 1])
        eps_temp = composed_mech.get_approxDP(delta)
        return abs(eps_temp-eps)

    return minimize_scalar(eps_from_c,bounds=[1e-8,1e2]).x

def eps_from_c2(c,
                frequency,
                forward_cnt,
                sigma,
                sigma_coeff=1.01,
                ):
    return np.exp(1/c**2)-1-frequency/forward_cnt*(np.exp(1/sigma**2)-np.exp(1/(sigma_coeff*sigma)**2))


def get_auto_sigma(
    epochs,
    batch_size,
    sample_size,
    frequency,
    epsilon,
    auto_lr=False,
    auto_noise=False,
    accountant='rdp',
    forward_cnt=3,
    sigma_coeff=1.01,
):
    delta = 1/sample_size
    sample_rate = batch_size/sample_size
    
    sigma = get_sigma(
            epochs,
            epsilon,
            delta,
            sample_rate,
            accountant=accountant
        )
    
    ####### get loss sigma based on sigma
    if auto_lr:
        # use auto_noise, adjust different budget for grad and loss
        if auto_noise:
            print("====> auto lr (w/ auto noise)")
            if accountant == 'rdp':
                our_sigma = find_c(epsilon, 
                               delta,
                               sigma,
                               epochs,
                               sample_rate,
                               forward_cnt,
                               frequency,
                               sigma_coeff=sigma_coeff
                               )
                sigma = sigma_coeff * sigma
            elif accountant == 'gdp':
                # our_sigma = fsolve(eps_from_c2,
                #                    sigma,
                #                    args=()
                #                    )[0]
                raise NotImplementedError
            else:
                raise ValueError

        # not auto-noise, use same budget for grad and loss
        else:
            print("====> auto lr (w/o auto noise) same noise for grad and loss")
            eps_epochs = (1 + forward_cnt / frequency) * epochs
            sigma = get_sigma(
                eps_epochs,
                epsilon,
                delta,
                sample_rate,
                accountant=accountant
            )
            our_sigma = sigma
    # no need for loss noise, only use priv grad
    else:
        print("====> no loss noise")
        our_sigma = None
    return sigma, our_sigma





import os
import lrfree
import wandb
import ml_swissknife.utils as ml_utils

from fastDP import PrivacyEngine
from torch.optim.lr_scheduler import LambdaLR

import torch
import torchvision
torch.manual_seed(2)
import torch.nn as nn
import torch.optim as optim
import timm
from opacus.validators import ModuleValidator
from opacus.accountants.utils import get_noise_multiplier
from tqdm import tqdm
import numpy as np
import warnings; warnings.filterwarnings("ignore")

from torch.optim.lr_scheduler import CosineAnnealingLR

'''Train CV with PyTorch.'''
def main(args):

    device= torch.device("cuda:0")
    # root=os.path.join(os.path.expanduser("~"), 'data')

    # Data
    transformation_resize224 = torchvision.transforms.Compose([
        torchvision.transforms.Resize((224,224)),#https://discuss.pytorch.org/t/runtimeerror-stack-expects-each-tensor-to-be-equal-size-but-got-3-224-224-at-entry-0-and-3-224-336-at-entry-3/87211/10
        torchvision.transforms.ToTensor(),
        torchvision.transforms.Normalize((0.5, 0.5, 0.5),(0.5, 0.5, 0.5)),
    ])
    # Define the transformations
    transform_1D = torchvision.transforms.Compose([
        torchvision.transforms.ToTensor(),
        torchvision.transforms.Normalize((0.5,), (0.5,))  # Normalize around the mean 0.5 and std 0.5
    ])
    if args.dataset_name in ['SVHN','CIFAR10']:
        num_classes=10
        transformation = transformation_resize224
    elif args.dataset_name in ['FashionMNIST']:
        num_classes = 10
        transformation = transform_1D
    elif args.dataset_name in ['CIFAR100','FGVCAircraft']:
        num_classes=100
        transformation = transformation_resize224
    elif args.dataset_name in ['Food101']:
        num_classes=101
        transformation = transformation_resize224
    elif args.dataset_name in ['GTSRB']:
        num_classes=43
        transformation = transformation_resize224
    elif args.dataset_name in ['CelebA']:
        num_classes=40
    elif args.dataset_name in ['Places365']:
        num_classes=365
    elif args.dataset_name in ['ImageNet']:
        num_classes=1000
    elif args.dataset_name in ['INaturalist']:
        num_classes=10000
        

    if args.dataset_name in ['SVHN','Food101','GTSRB','FGVCAircraft']:
        trainset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='train', download=True, transform=transformation)
        testset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='test', download=True, transform=transformation)
    elif args.dataset_name in ['CIFAR10','CIFAR100','FashionMNIST']:
        trainset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, train=True, download=True, transform=transformation)
        testset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, train=False, download=True, transform=transformation)
    elif args.dataset_name=='CelebA':
        trainset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='train', download=True, target_type='attr', transform=transformation)
        testset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='test', download=True, target_type='attr',transform=transformation)
    elif args.dataset_name=='Places365':
        trainset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='train-standard', small=True, download=True, transform=transformation)
        testset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='val', small=True, download=True, transform=transformation)
    elif args.dataset_name=='INaturalist':
        trainset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, version='2021_train_mini', download=True, transform=transformation)
        testset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, version='2021_valid', download=True, transform=transformation)
    elif args.dataset_name=='ImageNet':
        trainset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='train', transform=transformation)
        testset = getattr(torchvision.datasets,args.dataset_name)(root=args.root, split='val', transform=transformation)
        
    trainloader = torch.utils.data.DataLoader(
        trainset, batch_size=args.mini_bs, shuffle=True, num_workers=4)

    testloader = torch.utils.data.DataLoader(
        testset, batch_size=200, shuffle=False, num_workers=4)

    n_acc_steps = args.bs // args.mini_bs # gradient accumulation steps
    
    if args.auto_config:
        lr_adapter = lrfree.auto.LrAdapter_CV(args.configs, args.mini_bs)

    # Model
    if args.model in ['CNN']:
        from models.cnn import CNNModel
        net = CNNModel(num_classes=num_classes)
    else:
        net = timm.create_model(args.model, pretrained=True, num_classes = num_classes)
    
    if args.peft == 'lora':
        import peft
        config = peft.LoraConfig(r=8, target_modules=r".*\.mlp\.fc\d", modules_to_save=["head.fc"])
        net = peft.get_peft_model(net, config).to(device)
        net.print_trainable_parameters()
    elif args.peft == 'bitfit':
        for name,layer in net.named_modules():
            if hasattr(layer,'weight'):
                temp_layer=layer
        for name,param in net.named_parameters():
            if '.bias' not in name:
                param.requires_grad_(False)
            else:
                param.requires_grad_(True)
                print(f"Trainable bitfit params: {name}")
        for param in temp_layer.parameters():
            param.requires_grad_(True)
    net = ModuleValidator.fix(net).to(device)

    if args.dataset_name=='CelebA':
        criterion = nn.BCEWithLogitsLoss(reduction='none')
    else:
        criterion = nn.CrossEntropyLoss()
    
    if args.optim == 'SGD':
        optimizer = optim.SGD(net.parameters(), lr=args.lr)
    elif args.optim == 'AdamW':
        optimizer = optim.AdamW(net.parameters(), lr=args.lr)
    elif args.optim == 'Adam':
        optimizer = optim.Adam(net.parameters(), lr=args.lr)
    elif args.optim == 'prodigy':
        from prodigyopt import Prodigy
        optimizer = Prodigy(net.parameters(), lr=1., weight_decay=0.)
    elif args.optim == 'dadaptation':
        from dadaptation import dadapt_adam
        optimizer = dadapt_adam.DAdaptAdam(net.parameters(), lr=1.)
    else:
        raise ValueError
    
    if args.lr_decay == 'cos':
        cos_scheduler = CosineAnnealingLR(optimizer, T_max=10000, eta_min=1e-5)
    else:
        cos_scheduler = None
        

    if 'BiTFiT' in args.clipping_mode: # not needed for DP-BiTFiT but use here for safety
        for name,param in net.named_parameters():
            if '.bias' not in name:
                param.requires_grad_(False)

    # Privacy engine
    if 'nonDP' not in args.clipping_mode:
        sigma, our_sigma = lrfree.auto.get_auto_sigma(
            epochs=args.epochs,
            batch_size=args.bs,
            sample_size=len(trainset),
            frequency=args.lazy_freq,
            epsilon=args.eps,
            auto_lr=args.auto_config,
            auto_noise=args.auto_noise,
            accountant='rdp',
            forward_cnt=3,
            sigma_coeff=1.01
        )
        if our_sigma:
            lr_adapter.sigma = our_sigma
        if args.wandb:
            args.loss_sigma = our_sigma if our_sigma else 0
            args.grad_sigma = sigma
        print(f'adding noise level {sigma} | {our_sigma}')
        privacy_engine = PrivacyEngine(
            net,
            batch_size=args.bs,
            sample_size=len(trainset),
            noise_multiplier=sigma,
            epochs=args.epochs,
            clipping_mode='MixOpt',
            clipping_style='all-layer',
        )
        privacy_engine.attach(optimizer)       
        noise_multiplier = privacy_engine.noise_multiplier
    else:
        noise_multiplier = None 
    args.noise_multiplier = noise_multiplier
    
    def test(epoch):
        net.eval()
        test_loss = 0
        correct = 0
        total = 0
        with torch.no_grad():
            for batch_idx, (inputs, targets) in enumerate(tqdm(testloader)):
                inputs, targets = inputs.to(device), targets.to(device)
                outputs = net(inputs)
                if args.dataset_name=='CelebA':
                    loss = criterion(outputs, targets.float()).sum(dim=1).mean()
                else:
                    loss = criterion(outputs, targets);#print(loss.item())

                test_loss += loss.item()
                total += targets.size(0)
                if args.dataset_name=='CelebA':
                    correct += ((outputs > 0) == targets).sum(dim=0).float().mean()
                else:
                    _, predicted = outputs.max(1)
                    correct += predicted.eq(targets).sum().item()

            te_loss = test_loss/(batch_idx+1)
            te_acc = 100.*correct/total
            print(f'Epoch: {epoch} Test Loss: {te_loss:.3f} | Acc: {te_acc:.3f} ({correct}/{total})')

        net.train()
        return te_loss, te_acc
    
    def train(epoch):
        
        if args.lr_decay:
            assert args.optim != 'prodigy'
            if args.lr_decay == 'ln':
                lr_scale = 1 - epoch / args.epochs
                if not args.auto_config:
                    for g in optimizer.param_groups:
                        g['lr'] = g['lr'] * lr_scale
        else:
            lr_scale = 1.0

        net.train()
        train_loss = 0
        correct = 0
        total = 0
        tr_iter = iter(trainloader)
        train_loss_meter = ml_utils.AvgMeter()
        log_interval = len(trainloader) // args.eval_per_epoch
        scale = 1-epoch/args.epochs
        
        if epoch == 0 and args.auto_init:
            for param in net.parameters():
                if param.requires_grad:
                    param.previous = param.data.clone()
            
            # List of candidate learning rates
            if args.dataset_name == 'FashionMNIST':
                candidate_lrs = [1e-3, 5e-3, 1e-2, 5e-2, 1e-1]
            else:
                candidate_lrs = [1e-4, 5e-4, 1e-3, 5e-3, 1e-2]

            # Variable to track the best learning rate and its loss
            best_lr = None
            lowest_loss = float('inf')

            for batch_idx, (inputs, targets) in enumerate(trainloader):
                inputs, targets = inputs.to(device), targets.to(device)
                if batch_idx > 1:
                    break
                for lr in candidate_lrs:
                    # Set learning rate
                    for param_group in optimizer.param_groups:
                        param_group['lr'] = lr
                    
                    # Forward pass
                    outputs = net(inputs)
                    loss = criterion(outputs, targets)

                    # Backward pass
                    loss.backward()
                    optimizer.step()
                    optimizer.zero_grad()
                    
                    # update loss
                    outputs2 = net(inputs)
                    loss2 = criterion(outputs2, targets)

                    # Update the best lr based on loss
                    if loss2.item() < lowest_loss:
                        lowest_loss = loss2.item()
                        args.lr = lr
                        
                    # recover model parameters
                    for param in net.parameters():
                        if param.requires_grad:
                            param.data = param.previous

            for param_group in optimizer.param_groups:
                param_group['lr'] = args.lr

            print(f"Optimal initial learning rate: {args.lr} with loss {lowest_loss}")
   
        for batch_idx, (inputs, targets) in enumerate(tqdm(trainloader)):
            inputs, targets = inputs.to(device), targets.to(device)
            outputs = net(inputs)

            if args.dataset_name=='CelebA':
                loss = criterion(outputs, targets.float()).sum(dim=1).mean()
            else:
                loss = criterion(outputs, targets);#print(loss.item())

            loss.backward()
            if ((batch_idx + 1) % n_acc_steps == 0) or ((batch_idx + 1) == len(trainloader)):
                if args.auto_config:
                    if (batch_idx + 1) % (n_acc_steps * args.lazy_freq)==0:
                        lr_adapter.adjust(net, optimizer, n_acc_steps, tr_iter, device=device, scale=lr_scale) # DEFAULT
                        if 'nonDP' not in args.clipping_mode:
                            optimizer.original_step() # DP + auto lr
                        else:
                            optimizer.step() # Non-DP + auto lr
                    else:
                        optimizer.step() # Non-DP + auto lr
                else:
                    optimizer.step()
                    if cos_scheduler:
                        cos_scheduler.step()
                optimizer.zero_grad()     

            train_loss += loss.item()
            total += targets.size(0)
            if args.dataset_name=='CelebA':
                correct += ((outputs > 0) == targets).sum(dim=0).float().mean()
            else:
                _, predicted = outputs.max(1)
                correct += predicted.eq(targets).sum().item()
            train_loss_meter.step(loss.item())

            if (batch_idx+1) % log_interval == 0:
                te_loss, te_acc = test(epoch)
                if args.wandb:
                    log_dict = {
                        'lr': optimizer.param_groups[0]['lr'],
                        'tr_loss': train_loss_meter.item(),
                        'tr_acc': 100.*correct/total,
                        'te_loss': te_loss,
                        'te_acc': te_acc,
                        'loss_thre': lr_adapter.loss_thre if args.auto_config else 0,
                    }
                    wandb.log(log_dict)

        tr_loss = train_loss/(batch_idx+1)
        tr_acc = 100.*correct/total
        print(f'Epoch: {epoch} Train Loss: {tr_loss:.3f} | Acc: {tr_acc:.3f} ({correct}/{total})')
        
    if args.wandb:
        wandb.init(
        project='lrfree_v1',
        entity='rachelisapro',
        name=f'{args.dataset_name}_{args.model}_{args.optim}_eps{args.eps}_{args.wandb_suffix}',
        tags=args.wandb_tags,
        config=vars(args)
    )

    for epoch in range(args.epochs):
        train(epoch)
            # scheduler.step()
        # test(epoch)


if __name__ == '__main__':
    import argparse

    parser = argparse.ArgumentParser(description='PyTorch CIFAR Training')
    parser.add_argument('--lr', default=5e-4, type=float, help='learning rate')
    parser.add_argument('--epochs', default=5, type=int,
                        help='numter of epochs')
    parser.add_argument('--bs', default=1000, type=int, help='batch size')
    parser.add_argument('--mini_bs', type=int, default=250)
    parser.add_argument('--eps', default=-1, type=float, help='target epsilon')
    parser.add_argument('--dataset_name', type=str, default='CIFAR10',help='https://pytorch.org/vision/stable/datasets.html')
    parser.add_argument('--clipping_mode', type=str, default='MixOpt',choices=['BiTFiT','MixOpt', 'nonDP','nonDP-BiTFiT'])
    parser.add_argument('--model', default='vit_base_patch16_224', type=str, help='model name')
    parser.add_argument('--eval_per_epoch', default=10, type=int)
    
    parser.add_argument('--lr_decay', type=str, default=None, help='learning rate scheduler', choices=['ln', 'cos'])
    
    parser.add_argument('--peft', type=str, default=None, choices=['lora', 'bitfit'])
    parser.add_argument('--optim', default='Adam', type=str)
    parser.add_argument('--wandb', action='store_true')
    parser.add_argument('--wandb_suffix', default='', type=str)
    parser.add_argument('--wandb_tags', nargs='+', default=[])
    parser.add_argument('--auto_init', action='store_true', help="automatic initial lr")
    parser.add_argument('--auto_noise', action='store_true', help="turn on automatic dp accounting to adjust grad noise and loss grad")
    parser.add_argument('--lazy_freq', type=int, default=None)
    parser.add_argument('--auto_config', default=None, type=str, help="configuration file path for auto lr")
    parser.add_argument('--root', default=os.path.join(os.path.expanduser("~"), 'data'), type=str)

    args = parser.parse_args()
    
    if args.auto_config:
        args = lrfree.utils.set_config_args(args)
    if args.eps < 0:
        args.clipping_mode = "nonDP"
    main(args)

